On Assessing the Usefulness of Proxy Domains for Developing and Evaluating Embodied Agents

In many situations it is either impossible or impractical to develop and evaluate agents entirely on the target domain on which they will be deployed. This is particularly true in robotics, where doing experiments on hardware is much more arduous than in simulation. This has become arguably more so in the case of learning-based agents. To this end, considerable recent effort has been devoted to developing increasingly realistic and higher fidelity simulators. However, we lack any principled way to evaluate how good a "proxy domain" is, specifically in terms of how useful it is in helping us achieve our end objective of building an agent that performs well in the target domain. In this work, we investigate methods to address this need. We begin by clearly separating two uses of proxy domains that are often conflated: 1) their ability to be a faithful predictor of agent performance and 2) their ability to be a useful tool for learning. In this paper, we attempt to clarify the role of proxy domains and establish new proxy usefulness (PU) metrics to compare the usefulness of different proxy domains. We propose the relative predictive PU to assess the predictive ability of a proxy domain and the learning PU to quantify the usefulness of a proxy as a tool to generate learning data. Furthermore, we argue that the value of a proxy is conditioned on the task that it is being used to help solve. We demonstrate how these new metrics can be used to optimize parameters of the proxy domain for which obtaining ground truth via system identification is not trivial.

==> archive/ac_notes1.tex <==
\section{Andrea's notes}
\LP{are we integrating this into the paper?} Currently Def. 3 specifies a \textbf{total order} on simulators as
it orders them by a numerical score.

We slightly refine the definition to account for specific type of
errors, in an analogy to ``false positives'' and ``false negatives''
for object detectors.

For comparing agents we use what are called ``preference relations''. 

Given two agents, we have 4 possible outcomes:
\begin{enumerate}
\item $a>b$: agent $a$ is better than\textbf{ $b$;}
\item $a<b:$ agent $a$is worse than $b$;
\item $a\sim b$: (read: ``$a$ indifferent $b$''): agent $a$ has same
performance as $b$;
\item $a\Join b$: (read: ``$a$ incomparable $b$''): agent $a$ and
$b$ are incomparable.
\end{enumerate}
\medskip{}
\medskip{}
%
\begin{example}
[From metrics performance to agent preference relation]
\label{exa:metrics}Assume the partial order for the agent derives
from considering two scalar performance metrics $x$ and $y$ with
a certain tolerance $\delta$. 

For each performance metric there are 3 cases:
\begin{enumerate}
\item $|x_{b}-x_{a}|\leq\delta$: the performance of the two agents is indifferent
for the metric $x$. We write: ``$x_{a}\sim x_{b}$''. 
\item $x_{a}>x_{b}+\delta$: agent $a$ is better than $b$ at metric $x$.
\item $x_{b}>x_{a}+\delta$: agent $a$ is worse than $b$ at metric $x$.
\end{enumerate}
For two metrics there are 9 cases possible. The following table relates
the performance on the metrics to the preference relation on the agents:
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline 
 & $x_{a}>x_{b}$ & $x_{a}\sim x_{b}$ & $x_{a}<x_{b}$\tabularnewline
\hline 
\hline 
$y_{a}>y_{b}$ & $a>b$ & $a>b$ & $a\Join b$\tabularnewline
\hline 
$y_{a}\sim y_{b}$ & $a>b$ & $a\sim b$ & $a<b$\tabularnewline
\hline 
$y_{a}<y_{b}$ & $a\Join b$ & $a<b$ & $a<b$\tabularnewline
\hline 
\end{tabular}
\par\end{center}

Note the following:
\begin{itemize}
\item If $a>b$ then agent $a$ excels in at least one metric, and excels
or is indifferent for the others.
\item If $a\sim b$ then all the metrics are indifferent.
\item If $a\Join b$, then $a$ excels at one metric but $b$ excels the
other.
\end{itemize}
This construction generalizes easily to more metrics than 2.
\end{example}

\medskip{}

\medskip{}

We have constructed a preference relation on agents given the performance
metrics. Now we want to characterize the quality of a simulator.

We use the principle: ``The quality of a simulator (wrt some performance
metrics) is measured by its accuracy to guess the actual preference
relation on the agents induced by the metrics.''.

Rather than computing a scalar score, we can be more precise by classifying
the types of errors.

For an analogy, remember how errors are classified for a detector.
There are two outcomes: either the object is present, or it is absent.
Therefore, we can use a $2\times2$ table to consider all possible
scenarios:
\begin{center}
\begin{tabular}{|c|c|c|}
\hline 
 & object is present & object is absent\tabularnewline
\hline 
\hline 
detector says present & ok & false positive\tabularnewline
\hline 
detector says absent & false negative & ok\tabularnewline
\hline 
\end{tabular}
\par\end{center}

The off-diagonal entries are mistakes, and there are two types of
mistakes, called ``false negative'' and ``false positive''. 
As it turns out, there are 4 possible statistics but only 2 independent dimensions.

Therefore, detectors can be ordered with a partial order, because
there are 2 performance metrics: 
\[
(\text{false positives rate},\text{false negatives rate}).
\]

We adapt this analogy to our case. Recall that a preference relation
for agents wrt some metrics has 4 possible outcomes. The simulator
can guess any of those 4. Therefore, the analogous table is a $4\times4$
table:
\begin{center}
\begin{tabular}{|r|c|c|c|c|}
\hline 
in reality: & $a>b$ & $a\sim b$ & $a<b$ & $a\Join b$\tabularnewline
\hline 
\hline 
simulator guesses $a>b$ & ok & ? & ? & ?\tabularnewline
\hline 
simulator guesses $a\sim b$ & ? & ok & ? & ?\tabularnewline
\hline 
simulator guesses $a<b$ & ? & ? & ok & ?\tabularnewline
\hline 
simulator guesses $a\Join b$ & ? & ? & ? & ok\tabularnewline
\hline 
\end{tabular}
\par\end{center}

The off-diagonal are the mistakes. How can we classify the mistakes?

\medskip{}

\medskip{}

Here is a possible classification with mistakes classified in 3 classes (\ref{fig:errors}).

\begin{figure*}
\begin{tabular}{|r|c|c|c|c|}
\hline 
in reality: & $a>b$ & $a\sim b$ & $a<b$ & $a\Join b$\tabularnewline
\hline 
\hline 
simulator guesses $a>b$ & ok & \textcolor{olive}{overconfidence error} & \textcolor{purple}{error type 1} & \textcolor{purple}{error type 1}\tabularnewline
\hline 
simulator guesses $a\sim b$ & \textcolor{brown}{specificity error} & ok & \textcolor{brown}{specificity error} & \textcolor{brown}{specificity error}\tabularnewline
\hline 
simulator guesses $a<b$ & \textcolor{purple}{error type 1} & \textcolor{olive}{overconfidence error} & ok & \textcolor{purple}{error type 1}\tabularnewline
\hline 
simulator guesses $a\Join b$ & \textcolor{purple}{error type 1} & \textcolor{olive}{overconfidence error} & \textcolor{purple}{error type 1} & ok\tabularnewline
\hline 
\end{tabular}
\caption{\label{fig:errors}}
\end{figure*}

To follow the justification below, it is useful to keep in mind example~\ref{exa:metrics}.

These are the types of mistakes:
\begin{enumerate}
\item \textbf{\textcolor{purple}{Error type 1}}: The simulator has guessed
something that is in direct opposition to the reality. It implies
that it has switched the order for some metric. (For example in reality
$x_{a}<x_{b}$ but the simulator has concluded $x_{b}>x_{a}$.)
\item \textbf{\textcolor{brown}{Specificity error}}\textbf{: }In this case,
the simulator cannot find a difference between the agents for some
metric, although there is one. (For example, in reality $x_{a}>x_{b}$
but the simulator concluded $x_{a}\sim x_{b}$). These errors could
come from limited number of runs (assuming a ``simulator'' means
``running a simulator for $n$ runs'') from which it is not possible
to get statistically significant results.
\item \textbf{\textcolor{olive}{Overconfidence error}}: The simulator has
found a discrepancy when there isn't one. (For example, in actuality
$x_{a}\sim x_{b}$, but the simulator has found $x_{a}>x_{b}$). 
\end{enumerate}
Therefore, just like we can derive a partial order $(\text{false positives},\text{false negatives})$
for object detectors, we can derive a partial order for simulators
with the metrics
\[
(\text{errors type 1},\text{specificity errors},\text{overconfidence errors}).
\]

We an further refine this ordering by considering the impact of these
errors in the context of some task. 

Suppose that we are using the simulator to choose which agent to deploy
in reality. Then these are the consequences of each error:
\begin{itemize}
\item \textbf{\textcolor{purple}{Errors type 1}} and \textbf{\textcolor{brown}{specificity
error}}s: We might deploy a sub-optimal agent that does worse than
the optimal agent on some metric.
\item \textbf{\textcolor{olive}{Overconfidence error}}: No consequence:
when two agents had indifferent performance, the simulator has picked
an arbitrary one.
\end{itemize}



==> archive/ac_notes2.tex <==
\section{Being precise about the evaluation scenario}

Consider the Duckietown simulator that Anthony will remember for years to come in his dreams.
It is  parametrized by a constant $d>0$ corresponding to the time rendering interval. \footnote{Not the period of the observations, but rather the period that is useful to render frames from which the observations are computed.}
We call this \emph{the inaccuracy} of the simulator.
 Let $S(d)$ be the family of Duckietown simulators parametrized by rendering interval / inaccuracy.
What can we say about the family $S(d)$?

Let's make some assumptions: In principle $d\to 0$ corresponds to reality.
However, because the speed of the robot is bounded, there is a $d_0>0$ which we can call
the lower bound for physical realism. (Andrea had estimated this to be $d_0 = 1/(15\cdot 7)$.)
Lower than $d_0$, we are wasting computation. Higher than $d_0$, we are compromising accuracy for computation.

Which simulator in the family  $S(d)$ is the best with respect to the performance measure we established?

Here we should be very precise regarding exactly what is the evaluation scenario:
\begin{itemize}
    \item If we say "we will run simulation for 15 in-sim minutes", then of course a more accurate simulator wins. The optimal $d$ is $d_0$.
    \item However, if we say ``we will run a simulation for 15 reality minutes'' than we should take into account
            that $S(2 d_0)$ is much less accurate than $S(d_0)$, however we can run \emph{twice} the experiments with it.
\end{itemize}

In general we can think of many simulators that can be parametrized by accuracy measures like $d$; ranging from $d_0$ (highest $d$ that 
achieves reality simulation) to $\infty$ (a very inaccurate simulator).


Define the function $\rho(d) \in \mathbb{R}$ to be the ratio of in-sim time vs real time. $\rho=1$ means that we 
have real time simulation. $\rho= 20$ means that we can simulate 20 minutes in the real time of 1 minute. 

Assume that $\rho$ is monotone in $d$ (``more accurate takes more time'') so that $\rho(d_0)$ is very small (it takes 1 year to simulate 1 second)
and $\rho(\infty)$ is very large (we can simulate a million frames per second, if we are happy to simulate only a broken camera).

On the other hand, the ability for a simulator to rank agents is monotone increasing in the in-sim simulation time (more samples, better accuracy), and monotone decreasing with $d$ (getting more inaccurate). Suppose now we have a certain in-reality budget of $T$ seconds. Then we have $\rho(d)T$ simulation time.
Putting all in formulas we have
$$
 \text{accuracy}(d) = f(\text{sim time}, \text{sim inaccuracy}) = f( \rho(d) T, d).  
$$
We are now free to choose $d$. The prediction is [needs to make some obvious assumptions] is that in general $\text{accuracy}$ as a function
of $d$ is a concave function, which means that there is an optimal $d$, which also depends on the time budget.

We call $d^\star(T)$ \emph{the optimal budget-limited inaccuracy} (for a certain task).



\clearpage
\section{Are there other simulator performance measures?}

In this paper we use this idea:

\emph{A simulator is useful inasmuch as it allows to distinguish the performance of different agents on particular tasks.}

This seems totally cool; but is it the end of the story?

For example, in learning, one might have a different performance measure:

\emph{A simulator is useful inasmuch it helps to achieve efficient learning}

Is this measure the same or different than the previous measure?



==> archive/env_families.tex <==

% \LP{I think we can move up to ``Preliminaries'' the definition of the simulator family. We can also write down the problem of maximizing the ``usefulness'' or value for prediction. 
% \begin{equation}
%     \theta^*=\arg \min_\theta PETV(...)
% \end{equation}
% to make this nice we should define the PETV or RPETV as a function of simulator. 
% However in the case for learning we need to make that case that it can be useful to generate trajectories or rollouts from many different simulators in the family. As is the case in domain randomization. Therefore the usefulness of the simulator for learning should be in general evaluated over the family and not the single simulator instance. 
% }
\label{sec:env_families}
The metrics suggested in this paper can be used to optimize the usefulness of a proxy environment. It is relevant to define environment families to figure how optimization might improve their usefulness as well as what are the limitations of a given family. Simulators are usually used for such proxy environments so they will be used as an example of a proxy but the same concepts can be applied to a real environment. We make a distinction between a simulator instance (an instanciated simulator environment) and a simulator (A software that takes parameters as input and generate a parameterized simulator instance).

Using either of the Proxy Usefulness metrics (PPU, RPPU or LPU) defined previously, we can optimize the set of parameters $\theta$ of a simulator instance. We then denote $\theta^*_{M_i}$ for the optimal set of parameters for a simulator using the proxy usefulness metric $M_i$. Note that $\theta^*_{M_i} = \theta^*_{M_j}$ is certain only if ${M_i}$ and ${M_j}$ refer to the same metric (e.g. the perfect simulator according to RPPU may not be the perfect simulator according to LPU).

We define a family of simulator $\mathcal{F}(\theta)$ to be all the simulator instances that can be generated by sampling parameters $\theta \in \Theta$. We argue that a simulator family has a predefined discrepancy with the target environment that will not be reducible by optimizing the parameters $\theta$. By classifying simulators into families, it is possible to understand what are the limitations to the optimization procedure: in \cite{kadian2019making}, during the optimization of their simulation parameters, the authors found that the noise model was incorrect. This difference induces an environment discrepancy that is not reducible within the simulator family that is being optimized.

To find the most useful simulator instance within a family using a Proxy Usefulness metric and a simulator $S$, we need to find the set of parameters $\theta^*$ that maximizes the value of the surrogate environment. This can be written down as an optimization problem:

\begin{equation}
    \theta^*=\arg \min_\theta PU(S, \theta)
    \label{eq:opt_proxy_instance}
\end{equation}

In some other cases, we are interested in optimizing the simulator family itself. That is the case when domain randomization is used, and the parameters of the simulator instance $\theta$ are randomized. In this optimization problem, we want to tune the parameters that are offered as part of a simulator family, their ranges and possibly other non-parametric features of the simulator. The optimization problem is then posed as:

\begin{equation}
    S^*=\arg \max_S PU(S)
    \label{eq:opt_proxy_family}
\end{equation}

% \anc{Add note about computing resources. Should it be held fix ?}
% \anc{TODO: be more precise about task definition, DR, Data augmentation, etc. what is part of the sim, what is part of the task and what is part of the agent ?}


==> archive/generalizing_the_rg.tex <==
\section{Generalizing the Reality Gap}

The term reality gap is conflated and used to describe many different type of discrepancies between two environments.
The "Reality" part comes from the fact that controllers that suffers from the RG usually comes from simulation and are transferred to a real environment. The term "Gap" encapsulates all errors that are introduced during the transfer process.
Since our analysis is not limited to simulation to reality, and because it will not be restricted to the observation of errors between those environments, we will use the more precise term \textit{Env Transfer Value} (ETV), which describes how useful an environment is as a proxy for a second environment.
For this paper, an environment will either refer to a simulator or a real hardware embodiment. While a source (proxy) environment is usually a simulator and the target environment is usually the embodied setup, there is no requirements for the source to be a simulation and the target to be a real robot.
% Because the E2EV is a generalization of the reality gap, maximizing the E2EV may or may not result in a reduction of the reality gap, but reducing the reality gap will increase the E2EV.
\anc{was env-to-env value (E2EV) better ?}

==> archive/introduction.tex <==
% Template for new intro



Recent breakthroughs in machine learning have increased the popularity of data-driven approaches to solve tasks with embodied agents. As such, the value of data has increased dramatically. Obtaining data from robots is costly since it requires deployment of hardware, operation of the robot and time-consuming rollouts of policies. Moreover, the policy exploration process might end up in hardware damage while unsafe states are explored. For this reason, numerous works in robotics have been using proxy environments (referred to as source, substitute, or surrogate environments) as low-cost, low-fidelity representations of the target environment. By sacrificing fidelity, a proxy environment may offer multiple advantages: availability of ground-truth data such as robot localization, reduced cost of data collection,  ability to generate and randomize large numbers of samples, customization of scenarios to facilitate the learning of edge cases, parallelization of the data generation process, etc.


In the most common configuration, the source environment is a simulator and the target environment is a real robot, in which case the policy transfer is called "sim-to-real". However, it is also frequent to see "sim-to-sim" (\cite{james2019sim,golemo2018sim,yu2018policy}), or even "real-to-real", such as in the case of \cite{paull2017duckietown} where small, cheap robots are used to represent an expensive car, or in \cite{xia2019gibson} where authors used real-to-real to validate their sim-to-real performance. Our analysis of the environment discrepancies applies to all of these case, so we will use the more general term "env-to-env" for policy transfer.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/placeholder-image.png}
\caption{TODO}
\label{fig:intro}
\end{figure}


Any environment used as a proxy for a target environment introduces a set of discrepancies, often resulting in performance reduction. The ``reality gap'' is a term that is typically used in the context of sim-to-real, although the concept can be generalized to any environment transfer. For this reason, we will instead use the term ``environment gap'' \LP{what about ``domain'' instead of environment} as a more generic case.
The environment gap has been observed in multiple works, and the community has found multiple ways to mitigate its effects (i.e. "crossing the gap"), without actually explicitly quantifying it. As a result, algorithms that show good performance in some settings (e.g. when the environment discrepancy is small) may completely fail in others, and there are no methods of predicting transferability a priori.


In our work, we attempt to quantify the usefulness of a proxy environment by providing \textit{Proxy Usefulness} metrics. We analyze how the discrepancy between the environments have been previously quantified and how they impact the value of the proxy environment. We make a clear distinction between proxies used to predict task performance (used to select agents according to their performance) and data-generating proxies (used to generate data samples or policies). In the first case, we propose the \ac{RPPU}, a metric to quantify the predictivity of a proxy, enabling researchers to find the most predictive proxy available to them. 
%
We also prescribe a metric to assess the usefulness of a proxy to generate learning data or trained agents, also giving the possibility to researchers to compare different data-generating environments and select the one that yields the best agents.


Our new metrics allow robotics practitioners to tune some parameters of their proxy environment for which system identification is non-trivial and ground truth value for the target environment is often not available, such as observation blur, input delay, field of view, etc.
\LP{Let's be more clear about what we are specifically going to do to evaluate}
\LP{Should we have a claim of contributions?}

It is also possible that these new evaluation metrics can be backpropagated as an error signal into a differentiable simulation (e.g., \cite{Toussaint-RSS-18, differentiable_lcp_kolter} among many others) in order to maximize the value of a simulation as a proxy environment. \LP{If we aren't actually doing this maybe move to future work}

==> archive/related_work.tex <==
% Section about related work done by AnthonyC
%
%  Note for other available metrics described here:
%  https://www.evernote.com/shard/s618/sh/5b3e6d72-0861-f5f2-a71e-5598f8da3728/93b74bc71f6dfe08d4525322b46a46cb
%  Papers gets more in more close to what we are doing (last subsubsection is list of metrics for RG
% 


\section{Related work}

\subsection{Crossing the environment gap}
%We can remove the descriptions in the following paragraph to make it shorter
Multiple techniques exist to mitigate the effects of the environment gap. One such promising technique that has received a lot of attention lately is Domain Randomization \cite{peng2018sim,tobin2017domain,james2017transferring,muratore2019assessing}: during training, a different proxy is sampled from an environment family (see \ref{sec:env_families}) for each run, preventing the model from overfitting to a specific simulator.
In the best-case scenario, the target environment will appear as another sample from the same distribution. Data augmentation is another popular solution \cite{shrivastava2017learning, pashevich2019learning, bousmalis2017unsupervised} where a model is trained to augment data generated by a proxy to match that of the target environment.
Meta-learning and domain adaptation are also often used to transfer the knowledge acquired in a source domain to the target environment \cite{yu2018one, bousmalis2018using}, even if it is completely different \LP{how is it completely different?}.
\cite{mouret2013crossing, mouret201720} \LP{don't put cites in a sentence like this} show that it is possible to find which controllers are most likely to transfer well to the target setup using only a few sample experiments on the real robot, a method called ``The transferability approach''.
Crossing the gap was also shown to be possible by learning a common representation for both source and target environments in \cite{zhang2019adversarial}, where they impose a common state representation for environments using an autoencoder and a discriminator network. 
Alternatively, \cite{tzeng2020adapting} achieved a common representation by forming weakly aligned pairs of source and target data, effectively transferring the annotations to the target images.

\subsection{Optimizing the proxy}
In our work, we are more interested in the different ways to analyze the environment gap and improve the proxy rather than circumvent its effects. The first step to reduce the gap imposed by a proxy is to do proper system identification \cite{tan2018sim}. Some work has also been done to carry out tests to validate a proxy \cite{pepper2007robot} \LP{need more of a description than ``Some work''}. It is common \cite{chebotar2019closing,collins2020traversing,tan2016simulation,zhu2017model,klaus2012comparison,zagal2007combining} to use a task performance metric to optimize a proxy such as actuators gain, masses, static friction, etc. Recent papers have also shown success in improving their proxies by adding a module that learns inverse dynamics to adapt the action that the proxy outputs to the expected action in the target environment \cite{christiano2016transfer,hanna2017grounded}.

\subsection{Metrics to quantify the environments discrepancies}
Being able to quantify the environment gap may lead to better prediction of the transferability of agents. As such, multiple attempts have been made by the community to obtain a metric to quantify this gap. One specific work in that direction is \cite{koos2012transferability}, which establishes the sim-to-real disparity: a metric specific to an agent that predicts how well it will transfer to the real robot. By conducting only a few experiments both on the real robot and in simulation, it is possible to learn a surrogate model that will estimate the fitness function on the real robot via interpolation. However, it is assumed that we have access to a quick way to compute the distance between two controllers in a domain such that similar controllers will have a similar transferability (e.g. behavioral features), which is often not the case. Moreover, we are interested in a way to quantify the environment gap at the level of a simulator instead of at the agent level. We believe that the environment gap should be agnostic to the agent.

The ``v-gap'' \cite{vinnicombe1993frequency} \LP{what is the v-gap? should we write it down?} is another metric that has been used to quantify the discrepancy between robotic systems without any knowledge about their dynamics \cite{sorocky2020experience}. This metric compares two different controllers in a black-box fashion by measuring the Euclidean distance of their input-output response projected onto the Riemann sphere. By analyzing the input-output signals of two robotic systems, we can precisely define the v-gap. It is then possible to minimize it to find the most representative environment. This metric has the limitation of comparing only the dynamics and being only available for linear systems.

By using multiple simulators, \cite{cutler2014reinforcement} came propose a metric to define the fidelity of an environment $\Sigma_i$ to a target environment $\Sigma_j$. The fidelity is defined by the maximum error in the optimal value function. Using this metric, they can optimize the training of reinforcement-learning-based agents using multiple simulators, taking into account the cost of generating data for high-fidelity simulators. On the other hand, this definition is inconvenient when used to assess a simulator since the value function is not always trivially computed, especially in the real world. We believe that the definition of the environment gap should not be tightly coupled with machine learning, and it should be independent of the algorithm used.

In \cite{kadian2020sim2real}, the authors were able to create a high-fidelity virtual environment for their task using real-to-sim. Given agents and a task, they used the Pearson correlation coefficient between runs on the real robot and in simulation to evaluate the reality gap. This allowed them to find that the noise model for their dynamics was wrong and that learning-based agents were overfitting to the simulator environment by using glitches. In their work, they frequently refer to rank inversion to validate their empirical results, which is an idea that is also used in \cite{ligot2018mimicking}. Like the former, we support that the predictive ability of a simulator lay in its capacity to predict the performance ordering of the agents. In our work, we further define the environment gap based on rank inversion. Using a relative metric for the reality gap allows us to use multiple performance metrics to get an environment gap measure through partial ordering as shown in def. \ref{def:RPPU}.

\LP{connections to transfer learning?}
% First paragraph that we had from LP:
%In \cite{Koos_EC_2013}, the authors propose to estimate a transferability metric based on a simulation-to-reality disparity measure which is defined over robot behaviours. In this case evaluating the metric is likely as arduous as deploying directly onto the real robot in the first place. Another approach is the ``Sim2Real Correlation Coefficient'' \cite{kadian2019making}, which is defined as the Pearson correlation coefficient over ``accuracies'' in simulation and reality for $n$ methods. Analyzing the intermediate signals in Fig.~\ref{fig:agent-environment} is a commonly-used approach to evaluate the discrepancy in one of the components (e.g. to evaluate the dynamics error for manipulation \cite{collins2019quantifying}). However, this is myopic and does not consider the ways that different types of errors in the different components interact, nor does it necessarily correspond to a good metric of how useful the simulator is as a tool for learning. 
